The $\mathbf{P}$-Completeness of Inverted Index Traversal: On the Complexity of Evaluating Boolean Query DAGs

Modern AI agents increasingly rely on search infrastructure to execute complex, neuro-symbolic reasoning workflows. These workflows often compile into deeply nested, non-monotonic Boolean queries over text fields. However, standard query evaluation strategies over inverted indices face severe theoretical limits when handling these structures. Stateful iterator models (Document-at-a-Time) are structurally bounded by $\text{NC}^1$ formula evaluation, suffering a worst-case $O(2^{|Q|})$ exponential blowup in query complexity when unrolling re-convergent logic. Conversely, recursive materialization models (Term-at-a-Time) incur an $\Omega(|U|)$ space complexity penalty (the Universal Scan) when evaluating logical negation over the document universe. In this paper, we establish the theoretical boundaries of executing complex logic natively over an inverted index. We formalize a retrieval language ($\mathcal{L}_R$) based on Directed Acyclic Graphs (DAGs) and prove that its evaluation problem is strictly \textbf{$\mathbf{P}$-Complete}. To make evaluation tractable, we introduce \texttt{ComputePN}, a deterministic, sparsity-aware evaluation algorithm. By decoupling logical negation from universe-scale materialization via a novel Positive-Negative dual representation, and utilizing native DAG memoization, \texttt{ComputePN} strictly bounds evaluation time to $O(|Q| \cdot |U_{\mathit{active}}|)$. This approach successfully evaluates $\mathbf{P}$-Complete queries natively over the index, avoiding both the combinatorial tree-expansion bottleneck and the universal scan penalty, laying the formal foundation for computational retrieval.

==> 7.tex <==
\section{A Computational Retrieval Architecture}
\label{sec:architecture}

The theoretical results ($\mathbf{P}$-Complete Evaluation) and algorithmic advances (\texttt{ComputePN}) presented in this paper unlock a new architectural pattern for information systems: \textbf{Computational Retrieval}. While traditional relational databases excel at structured logic and standard search engines excel at unstructured semantic ranking, modern AI applications require the seamless integration of both.

In this proposed architecture, the retrieval engine ceases to be a simple document filter; it functions as a logic co-processor that unifies precise Boolean execution with soft semantic ranking. The Large Language Model (LLM) serves as an \textbf{Intelligent Gateway}, leveraging its internal world knowledge and immediate user context to bridge the gap between vague natural language and precise retrieval constraints. 

Unlike standard workflows where the LLM reacts to broad search results (``Fetch-then-Filter''), here the LLM proactively resolves ambiguities---mapping synonyms, inferring date ranges, and identifying entities---and \textit{compiles} that understanding into a precise Query DAG. The \texttt{ComputePN} engine then acts as the low-level \textit{Executor}, enforcing these constraints directly over the index structure without data movement, before passing the logically valid candidates to a downstream ranker.

\subsection{Theoretical Implications: The Index as a CPU}
One implication of Corollary~\ref{cor:PComplete} is that the retrieval engine can be interpreted as a broader computational substrate. Because $\mathcal{L}_R$ is descriptively equivalent to polynomial-size propositional circuits, the engine is no longer restricted to evaluating strict syntactic trees ($\text{NC}^1$). Theoretically, the LLM can compile bounded arithmetic operations natively into a re-convergent Query DAG, provided the underlying numerical fields (e.g., Year, Citations) are indexed in a binary-decomposed format. In this view, the inverted index functions as a massively parallel SIMD memory~\cite{flynn1972some}, utilizing bit-sliced arithmetic~\cite{oneil1997quasidistributed} to execute numerical operations across billions of documents in a single pass.

It is worth noting that while query languages like SQL with Recursive CTEs are Turing Complete (when combined with arithmetic operations~\cite{abiteboul1995foundations}), such expressiveness is a liability for high-performance retrieval. Turing completeness means the system cannot provide any theoretical guarantee on execution time, creating the risk of unbounded processing as data scales.

By defining $\mathcal{L}_R$ strictly as a language of acyclic graphs, we enforce a hard upper bound on computational complexity. This represents an attractive tradeoff between expressiveness and predictability: the language is expressive enough to simulate the bounded propositional circuits (e.g., adders, comparators) required for neuro-symbolic reasoning, yet structurally guarantees termination and optimal $\mathcal{O}(|V| \cdot |U_{\mathit{active}}|)$ runtime. This ensures the retrieval engine functions as a predictable, high-throughput accelerator, maintaining polynomially bounded execution times regardless of the depth of the reasoning task.

\subsection{Integration with Ranking Pipelines}
\label{subsec:ranking}
Our architecture explicitly incorporates ranking to prioritize logically valid candidates. In scenarios where the Boolean result set remains large, the Planner utilizes a \textbf{Dual-Payload Protocol}, issuing a composite request $\langle Q_{DAG}, Q_{Rank} \rangle$.

\noindent \textbf{The Dual-Payload Execution:} The Planner constructs a bifurcated Query Execution Plan (QEP) consisting of strict retrieval logic ($Q_{DAG}$) and soft ranking signals ($Q_{Rank}$). \texttt{ComputePN} executes $Q_{DAG}$ to produce the precise candidate set $S_{valid}$ in polynomial time. Subsequently, the ranking module utilizes $Q_{Rank}$ to compute final relevance scores strictly over $S_{valid}$. This scoring phase can seamlessly integrate lexical metrics (e.g., BM25), semantic embedding distances (e.g., Cosine Similarity), and behavioral priors (e.g., user engagement signals or click-through rates). This ensures the top results are not just prioritized by multi-modal utility, but are mathematically guaranteed to satisfy the logical boundaries of the user's request.

\noindent \textbf{Offloading Logic from Deep Re-rankers:} Modern search architectures frequently employ a final, computationally intensive re-ranking stage using deep neural models (e.g., Cross-Encoders) to maximize semantic precision. However, these models are not designed to provide formal guarantees regarding strict logical constraints~\cite{weller2025theoretical}. Furthermore, because their inference cost scales linearly with the number of candidates, evaluating them over broad, unfiltered result sets is practically infeasible. \texttt{ComputePN} acts as a strict logical firewall at the very beginning of the pipeline. By enforcing the constraints during the initial, highly efficient retrieval phase, it ensures that the expensive downstream rankers consume compute resources \textit{only} on logically valid candidates, thereby maximizing the utility of the available inference budget while guaranteeing strict compliance with the agent's intent.


==> CollectConsecutiveIntervals.tex <==
\section{Implementation of CollectConsecutiveIntervals}\label{secCollectConsecutiveIntervals}

The \texttt{CollectConsecutiveIntervals} function is a helper utility designed to efficiently identify maximal consecutive sequences of document IDs within a node's result set. It plays a particularly important role in correctness of the Negation Nodes within our Boolean retrieval system.

  Given a leaf node $n$, this function identifies the longest consecutive interval of document IDs,  $\langle f, l\rangle$, that satisfies the following conditions:

  \begin{enumerate}
    \item $f$ is equal to the document ID currently pointed to by $n.\text{State.Ptr.ID}$;
    \item For every document ID $d$ such that $f \le d \le l$, $d$ must be present in $n$'s underlying posting list;
    \item Document ID $l+1$ is not present in $n$'s underlying posting list.
  \end{enumerate}

  A key characteristic of \texttt{CollectConsecutiveIntervals} is that it does not modify the internal state or advance the document ID pointer of the node $n$ upon which it operates. Its sole responsibility is to report the bounds of the identified consecutive block.

\begin{algorithm}[H]
\caption{CollectConsecutiveIntervals($n$)}\label{algCollectConsecutiveIntervals}
\begin{algorithmic}[1]
\Function{CollectConsecutiveIntervals}{$n$} 
    \State $currentPtr \gets n.\text{State.Ptr}$
    \If{$currentPtr = \text{nil}$} \Comment{If node is exhausted or empty}
        \State \Return $\Call{MakeInterval}{U+1, U}$ 
    \EndIf

    \State $f \gets currentPtr.\text{ID}$ 
    \State $l \gets currentPtr.\text{ID}$ 
    \State $tempPtr \gets currentPtr.\text{Next}$

    \While{$tempPtr \ne \text{nil}$ \textbf{and} $tempPtr.\text{ID} = l + 1$}
        \State $l \gets tempPtr.\text{ID}$
        \State $tempPtr \gets tempPtr.\text{Next}$
    \EndWhile
    \Return $\Call{MakeInterval}{f, l}$
\EndFunction
\end{algorithmic}
\end{algorithm}

  It's worth noting that while Algorithm~\ref{algCollectConsecutiveIntervals} illustrates the logic using a conceptual linked list representation of a posting list, real-world implementations often utilize flat arrays or linked lists of arrays for posting lists. In such array-based scenarios, the process of finding the longest consecutive interval (i.e., determining $l$) can be further optimized by employing binary search within these arrays, significantly improving performance for large posting lists.

==> Expressiveness.tex <==
\section{A Framework for High-Precision Search and its Expressive Power}\label{secExpressivePower}

    This section first describes the two main components of our proposed framework: an offline process for semantic data enrichment and an online engine for real-time query execution. We then formally analyze the expressive power of this framework's retrieval language, proving that it captures the complexity class \textbf{P}. This result establishes a link between logical expressiveness and computational complexity for retrieval, in the spirit of the celebrated Immerman-Vardi theorem which forged a similar connection for relational databases~\cite{immerman1986relational,vardi1982complexity}.

    \subsection{Architectural Context}\label{subsecFramework}
        Our framework's practical utility is realized in a two-stage process. The core theoretical results apply to an online retrieval engine that executes formal queries. We assume this engine operates on a rich index generated by an offline process.

        This offline process is responsible for creating a structured, field-based index from raw documents. We assume this index is augmented with rich metadata, which can be derived from various sources such as human curation, external knowledge bases (e.g., DBLP), or model-based entity and fact extraction. The specific origin of these features is less important than their existence, as they form the atomic propositions over which our logical language operates.

        With a richly annotated index in place, the online component handles user queries in real-time. This stage bridges the gap between natural language and formal logic in two steps: (1) \textit{Query Understanding}, where an LLM translates the user’s input into a Query DAG, using techniques like chain-of-thought prompting~\cite{wei2022chain} and constrained decoding~\cite{shin2021constrained}; and (2) \textit{Logical Execution}, where the \texttt{ComputePN} algorithm (Section~\ref{secProposedApproach}) executes the DAG with high efficiency and guaranteed precision. This proposed synergy represents the architectural vision for next-generation precision search.

    
        %While our retrieval engine is designed to execute precise, complex Boolean queries, its practical utility is maximized when placed within a broader system. To this end, we propose a retrieval framework that addresses two key challenges: the difficulty for users to formulate complex queries and the need for rich, underlying data. This proposed framework is composed of two complementary stages.
        
        %\subsubsection{Offline Pre-processing: Data Structuring and Enrichment}
        %The power of our expressive query language is only fully realized when it operates on a detailed and structured index. Therefore, the foundational offline stage of our framework consists of two phases: first structuring the raw data, and then enriching it with additional semantic metadata.
        
        %\textbf{1. Document Processing and Structuring.} Initially, each document in the corpus—whether unstructured (plain text), semi-structured (HTML, Academic Papers), or structured (a database record)—is processed into a consistent, field-based format. For an academic paper, this involves parsing the raw file (e.g., a PDF) to extract and demarcate standard fields like \texttt{TITLE}, \texttt{AUTHORS}, \texttt{ABSTRACT}, and \texttt{REFERENCES}. This step ensures that all documents have a common schematic base upon which enrichment can be built.
        
        %\textbf{2. Metadata Enrichment and Augmentation.} Once the documents are structured, we augment them with a deeper layer of queryable metadata. This enrichment process adds valuable features that may not be explicit in the original document:
        %\begin{itemize}
        %    \item \textbf{Human Curation:} An editorial team can add high-quality labels, such as normalizing author affiliations or assigning official conference keywords.
        %    \item \textbf{External Data Integration:} The structured data is linked with external knowledge bases like DBLP or Semantic Scholar to import additional features, such as citation counts, author h-indexes, or associated datasets.
        %    \item \textbf{Model-Based Extraction:} Modern language models are used to infer abstract properties from text of the paper. For example, a model can read the paper and generate structured tags like \texttt{METHOD:transformer}, \texttt{TASK:question-answering}, \texttt{CONTRIBUTION:theoretical} or \texttt{BENCHMARK:SQUAD}.
        %\end{itemize}
        
        %The final output of this offline pipeline is a collection of documents annotated with a rich, multi-faceted set of field-qualified tokens. This creates the high-fidelity index required for our online engine to answer sophisticated queries.
        
        %\subsubsection{Online Retrieval Engine} With a richly annotated index in place, the online component handles user queries in real-time. This stage bridges the gap between natural language and formal logic in two steps: (1) \textit{Query Understanding}, where an LLM translates the user's input into a Query DAG, using techniques like chain-of-thought prompting \cite{wei2022chain} and constrained decoding \cite{shin2021constrained}; and (2) \textit{Logical Execution}, where our \texttt{ComputePN} algorithm (Section~\ref{secProposedApproach}) executes the DAG with high efficiency and guaranteed precision. This proposed synergy represents our architectural vision for next-generation precision search.

    \subsection{Expressive Power of the Retrieval Language}\label{subsecExpressivePower}
        Having defined our framework, we now formally analyze the expressive power of its underlying retrieval language. The ability of our system to represent any query as a \textbf{Query DAG} using the functionally complete operator set {\texttt{AND}, \texttt{OR}, \texttt{NOT}} \cite{enderton2001mathematical,sipser2012introduction} allows it to express any logical condition over the indexed features.

        To formalize our framework's capabilities, we define a Boolean function, \texttt{Retrieve($\mathcal{I}, Q$)}, which takes an \textbf{Index}, $\mathcal{I}$, and a general \textbf{Query DAG}, $Q$. The function operates by first transforming $Q$ into its equivalent Normalized Query DAG, $Q_N$, and then returns \textbf{True} if executing our \texttt{ComputePN} algorithm on $\langle \mathcal{I}, Q_N \rangle$ yields a non-empty result, and \textbf{False} otherwise. This \texttt{Retrieve} function is the characteristic function for our \textbf{Retrieval Language}, $\mathcal{L_R}$, which we define as the set of all input pairs $\langle \mathcal{I}, Q \rangle$ that evaluate to True. With these formalisms, we can state our primary theoretical result:

        \begin{theorem} \label{propExpressiblity}
            The Retrieval Language $\mathcal{L_R}$ precisely \textbf{captures} the complexity class \textbf{P}.
        \end{theorem}

        To prove Theorem~\ref{propExpressiblity}, we must show the following two conditions are met~\cite{immerman1999descriptive}: (1) the decision problem for our language is solvable in polynomial time, and (2) any problem in \textbf{P} can be reduced to our decision problem via a LogSpace reduction.

        The first condition is met because our \texttt{Retrieve} function is composed of two polynomial-time stages: DAG normalization, which is polynomial in the size of the query, and the execution of the \texttt{ComputePN} algorithm, which is polynomial in the size of the query and the index.

        To satisfy the second condition, we demonstrate a LogSpace reduction from the canonical \textbf{P}-complete problem, the Circuit Value Problem (CVP) \cite{ladner1975circuit,arora2009computational}. We construct an instance $\langle \mathcal{I}, Q\rangle$ from a given CVP instance $\langle C, A\rangle$ as follows:

        \begin{enumerate}
            \item \textbf{Construct the Index, $\mathcal{I}$:} We create a minimal collection with a single document, $D_{true}$, and a single token, `Truth`. The posting list for `Truth` is $\{D_{true}\}$.
        
            \item \textbf{Construct the Query DAG, $Q$:} We transform the circuit $C$ into a Query DAG. Gates map to their corresponding node types. An input wire assigned \textbf{True} becomes a Leaf node for `Truth'; an input wire assigned \textbf{False} becomes a `NOT' node with a `Truth' Leaf child.
        
            \item \textbf{Conclusion:} The original CVP instance is True if and only if \texttt{Retrieve}($\mathcal{I}, Q$) returns True.
        \end{enumerate}

        The correctness of this transformation follows by induction on the structure of the circuit. The \textbf{base cases} (the input wires) correctly map the circuit's True/False values to our system's non-empty/empty result sets. The \textbf{inductive step} holds because the query nodes for \texttt{AND}, \texttt{OR}, and \texttt{NOT} directly mirror the semantics of their corresponding logic gates.
        
    \subsection{Implications and Vision}
        Our finding that the retrieval language captures \textbf{P} has profound implications, moving our system beyond simple keyword matching into the realm of computational retrieval. This result establishes that our framework's expressive power is not limited to set-based Boolean logic, but extends to \textbf{evaluating complex arithmetic and numerical constraints} over indexed features. This capability is analogous to foundational results in database theory \cite{immerman1986relational,vardi1982complexity} and provides a significant advantage over embedding-based systems, which struggle with precise logical and numerical reasoning~\cite{Rossi_2024,zhang2024boolquestions,karpukhin2020dense}.

        The ability to encode P-time computable properties as a Query DAG means we can construct queries for sophisticated numerical conditions. These examples demonstrate that by supporting general DAG structures and full negation, our engine can perform computations far beyond simple keyword retrieval.

        \begin{compactenum}
            \item \textbf{Strong Negation with High Selectivity:} Consider a query like ``recent papers in NLP that are NOT used deep learning.'' An LLM-based agentic framework would likely decompose this into a slow, multi-step ``fetch-then-filter'' process. In contrast, our framework excels. The entire query is resolved in a single, efficient pass over the index. This demonstrates how our engine handles strong negations as a native, low-latency operation, avoiding the costly iterative filtering required by agentic workflows.
            \item \textbf{Parity Checks:} A query for ``papers with an odd number of keywords from a list'' can be implemented by building a parity-checking circuit from a cascade of XOR gates. A tree-based query for this would be exponential in size, while our DAG representation is linear, $O(k)$, where $k$ is the number of authors.
            \item \textbf{Thresholding and Counting:} A query for ``papers written by at least $k$ of a given $N$ authors'' can be modeled by constructing a circuit of binary adders (or simulating the dynamic programming computation) within the Query DAG to count the matching authors.

            \item \textbf{Numerical Comparison:} A query for ``papers cited more than $K$ times'' is enabled by indexing citation counts in a binary format (e.g., \texttt{CITE\_BIT\_0:true}). The Query DAG then implements a digital comparator circuit to check if a document's citation number is greater than $K$.

        \end{compactenum}
        
        The capabilities demonstrated in these examples—from efficiently handling strong negations to performing complex numerical comparisons—point to a crucial architectural insight: a search index can be queried like a computational circuit. This positions our framework as an essential high-performance fast path for modern multi-agent search systems. This creates a clear operational model:


        \begin{compactitem}
            \item \textbf{The Fast Path (Our Framework):} An LLM planner identifies that a query, even if complex or arithmetic-heavy, can be resolved entirely against the pre-computed index. It then translates the query into a single Query DAG, targeting our engine for fast, single-pass execution. This path excels at tasks like the ``Strong Negation'' query, replacing a slow, iterative agentic filtering process with a native, low-latency logical evaluation.


            \item \textbf{The Complex Path (Escalation):} Only queries that cannot be resolved against the index alone need to be escalated to the slower, multi-tool agentic pipeline. This applies to tasks requiring:
            \begin{compactitem}
                \item Real-time external data (e.g., ``authors whose citation count grew last month'').
                \item Unconstrained natural language generation (e.g., ``summarize this paper's findings'').
                \item Access to facts not present in the pre-computed index.
            \end{compactitem}
            
        \end{compactitem}
        
        In this vision, our work provides a robust and tractable engine that carves out a vast new class of computational queries that can be moved off the expensive, high-latency reasoning path. It reserves true agentic delegation for the small fraction of requests that genuinely require it.

        

==> MusicQueryTrees.tex <==
\section{A Case Study: Music Search with Complex Queries}\label{secCaseStudy}
    To demonstrate the practical utility of support for complex queries in retrieval, this section presents a case study of a hypothetical music search engine. We showcase how our proposed Boolean query evaluation can handle sophisticated, real-world user queries that are challenging for standard retrieval systems.

    For this case study, we assume the search engine uses a standard inverted index built from a large corpus of songs. Each song's metadata (e.g., \textit{Title}, \textit{Artists}, \textit{Genres}) is indexed using field-qualified unigrams. For example, the title ``Yellow Submarine'' would produce the tokens \texttt{TITLE:yellow} and \texttt{TITLE:submarine}, in addition to the raw tokens \texttt{yellow} and \texttt{submarine}. This field-aware tokenization allows for precise, targeted queries.
    \subsection{Complex Queries for Music Search}\label{subSecComplexQueries}
        This subsection presents several natural language queries and their corresponding translations into complex Boolean Query Trees. These translations were generated using Google's Gemini Pro to illustrate how a modern LLM can act as a sophisticated ``Query Understanding'' module. 
\begin{longtable}{>{\raggedright\arraybackslash}p{5cm} | >{\raggedright\arraybackslash}p{6cm}}
\caption{Examples of queries and their Query DAG.}
\label{tab:query_examples} \\

% --- HEADER for the FIRST page ---
\hline
\textbf{Natural Language Query} & \textbf{Generated Boolean Query DAG} \\
\hline
\endfirsthead

% --- HEADER for ALL SUBSEQUENT pages ---
\hline
\multicolumn{2}{|l|}{\tablename\ \thetable\ -- \textit{Continued from previous page}} \\
\hline
\textbf{Natural Language Query} & \textbf{Generated Boolean Query DAG} \\
\hline
\endhead

% --- FOOTER for all pages EXCEPT THE LAST ---
\hline \multicolumn{2}{r}{{\textit{Continued on next page}}} \\
\endfoot

% --- FOOTER for THE LAST page ---
\hline
\endlastfoot

% --- TABLE CONTENT ---

% --- ROW 1 ---
\textit{Songs by Young Blood} & \vspace{-1.2em}\lstinputlisting{query1.txt} \\ \hline

% --- ROW 2 ---
\textit{Show me songs by Taylor Swift, but exclude any of her country tracks.} &
\vspace{-1.2em}\lstinputlisting{query2.txt} \\ \hline

% --- ROW 3 ---
\textit{Find songs featuring Beyoncé and JAY-Z, but not if Drake is also on the track.} &
\vspace{-1.2em}\lstinputlisting{query3.txt} \\ \hline

% --- ROW 4 ---
\textit{Give me Electronic music that is either Ambient or Chillwave, but absolutely no Dubstep.} &
\vspace{-1.2em}\lstinputlisting{query4.txt} \\ \hline

% --- ROW 5 ---
\textit{Songs about love or happiness, but specifically not break-up songs or tracks with a sad mood.} &
\vspace{-1.2em}\lstinputlisting{query5.txt} \\ \hline

% --- ROW 6 ---
\textit{Classic 80s Rock songs, but not from those cheesy ``hair bands."} &
\vspace{-1.2em}\lstinputlisting{query6.txt} \\ \hline

\end{longtable}


  As these examples illustrate, some complex queries, particularly those involving nuanced exclusions (e.g., Items 3, 4, 5, and 6), pose significant challenges for purely embedding-based retrieval systems. Such systems often yield numerous irrelevant results (false positives) for these specific types of queries, highlighting the precision advantage  of Boolean query trees. 

==> Proofs.tex <==
\section{Proofs}\label{secProofs}
    \begin{proposition}
        Every Query Tree can be transformed into an equivalent Normalized Query Tree.    
    \end{proposition}

   
   \begin{proof} Given an arbitrary Query Tree, we can convert it into an equivalent Normalized Query Tree by applying the following transformations iteratively: 
        \begin{enumerate}
            \item \textbf{Simplifying Empty Terms:} 
                    Every Leaf Node corresponding to an empty posting list is replaced with a $False$ literal. The tree is then simplified by applying standard boolean algebra rules (e.g., absorbing \texttt{False} in \texttt{AND} operations, eliminating \texttt{False} in \texttt{OR} operations, and converting \texttt{NOT False} to \texttt{True}, etc).
            \item \textbf{Pushing Down Negations:} For any \texttt{NOT} node whose child is not a \texttt{Leaf Node}, we push the negation down the tree using De Morgan's Laws and the double negation elimination rule . This process is applied iteratively until all \texttt{NOT} nodes are direct parents to \texttt{Leaf Nodes}.

            \item \textbf{Normalizing Branching Factor of AND and OR Nodes:} 
                \begin{itemize}
                    \item \textbf{Handling Single Child:} Any \texttt{AND} or \texttt{OR} node with only one child is removed and replaced by its child.
                    \item \textbf{Handling Multiple Children:} Any \texttt{AND} or \texttt{OR} node with more than two children is transformed into a binary sub-tree using associativity.
                \end{itemize}
                These transformations are applied iteratively until all \texttt{AND} and \texttt{OR} nodes have exactly two children.
        \end{enumerate}     
    \end{proof}


==> PropMethod.orig.tex <==
\subsection{Complexity Analysis (Sparsity Guarantee)}
We now prove that \texttt{ComputePN} evaluates $\mathcal{L}_R$ in polynomial time with respect to the \textbf{active data}, ensuring strict sparsity-awareness. Furthermore, we demonstrate that the algorithm can be partitioned to operate within any strict auxiliary memory bound $M$.

\begin{theorem}[Time and Space Complexity]\label{thm:computepn_complexity}
Let $Q$ be a Query DAG with $|V|$ nodes. Let $U_{\mathit{active}} = \bigcup_{t \in \text{leaves}(Q)} \mathcal{I}(t)$ be the union of all document IDs referenced by terms in $Q$. Given any auxiliary memory bound $M \ge |V|$, \texttt{ComputePN} can evaluate $Q$ with a space complexity of $\mathcal{O}(M)$ and a time complexity of $\mathcal{O}(|V| \cdot |U_{\mathit{active}}|)$.
\end{theorem}

\begin{proof}
We first observe a fundamental invariant of the PN-Algebra defined in Section~\ref{subsec:PNComputeEvaluation}: none of the algebraic rules introduce new document IDs into the materialized set $S_v$ that were not present in the children.
\begin{itemize}
    \item \textbf{Leaf Nodes:} $S_{leaf} \subseteq U_{\mathit{active}}$ by definition.
    \item \textbf{Negation ($\neg$):} The operation $\langle S_C, T_C \rangle \to \langle S_C, \neg T_C \rangle$ preserves the materialized set exactly ($S_v = S_C$). Thus, if $S_C \subseteq U_{\mathit{active}}$, then $S_v \subseteq U_{\mathit{active}}$.
    \item \textbf{Binary Operators ($\land, \lor$):} Operations $S_L \cup S_R$, $S_L \cap S_R$, and $S_L \setminus S_R$ all produce results that are subsets of $S_L \cup S_R$. Even in the critical case of Disjunctive Negation (e.g., $A \cup \neg B \to \neg(B \setminus A)$), the materialized set is $B \setminus A$, which is a subset of $B$, and thus a subset of $U_{\mathit{active}}$.
\end{itemize}
By induction, for any node $v$, $S_v \subseteq U_{\mathit{active}}$. Therefore, $|S_v| \le |U_{\mathit{active}}|$. 

To satisfy the memory bound $M$, the algorithm employs a Block-at-a-Time (BAAT) partitioning strategy, a technique established in high-performance retrieval systems~\cite{moffat1996self, ding2011faster}. The active domain $U_{\mathit{active}}$ is partitioned into disjoint blocks of maximum size $B = \lfloor M / |V| \rfloor$. Because $M \ge |V|$, $B \ge 1$.

The algorithm evaluates the entire DAG $Q$ strictly within the boundaries of a single block. Because the materialized set $S_v$ for any node is bounded by the block size $B$, the memoization table requires at most $|V| \cdot B \le M$ auxiliary space. Once a block is evaluated, the memoization table is flushed, and the algorithm proceeds to the next block.

The time cost to evaluate a single node over a block of size $B$ is $\mathcal{O}(B)$. The time to evaluate the entire DAG over one block is $\mathcal{O}(|V| \cdot B)$. Because there are $\lceil |U_{\mathit{active}}| / B \rceil$ blocks, the total time complexity is:
\[ \mathcal{O}\left( \frac{|U_{\mathit{active}}|}{B} \cdot |V| \cdot B \right) = \mathcal{O}(|V| \cdot |U_{\mathit{active}}|) \]
Thus, the algorithm strictly respects the memory bound $M$ while maintaining the optimal time complexity. This time complexity matches the theoretical lower bound of the problem, as any evaluation algorithm must inspect the query graph of size $|V|$ and the active data elements of size $|U_{\mathit{active}}|$.
\end{proof}

\noindent \textbf{Significance and Data-Parallel Execution:} 
Theorem~\ref{thm:computepn_complexity} establishes that \texttt{ComputePN} scales strictly with the information content of the query ($|U_{\mathit{active}}|$), maintaining tractability even as the collection size $|U|$ grows to billions of documents. Furthermore, because the block partitions $P_i$ are strictly disjoint, the evaluation is embarrassingly parallel. Given a multi-core architecture, the engine can evaluate $c$ blocks concurrently. 

While modern DAAT engines also utilize index sharding to achieve data-parallelism, they remain mathematically bound by the $\Omega(2^{c|Q|})$ Tree-Expansion bottleneck (Theorem~\ref{thm:daat_rewrite_lower}) within each shard. In contrast, \texttt{ComputePN} uniquely achieves data-parallel scalability while strictly maintaining $O(|Q|)$ query complexity and $O(|U_{\mathit{active}}|)$ space complexity per shard, making it the only viable architecture for distributed neuro-symbolic retrieval.

\subsection{DAG Optimization and Rewriting}
Because our execution model operates on an explicit data structure (the Query DAG) rather than an opaque iterator stack, we can apply a suite of \textbf{structural and data-aware optimizations} to minimize computational cost before the heavy lifting of intersection begins.

\begin{itemize}
    \item \textbf{Common Subexpression Elimination (CSE):} If the input query structure contains repeated sub-expressions (e.g., duplicating a complex date filter across multiple branches), the engine detects and merges these identical sub-graphs. This automatically transforms a redundant syntactic tree into a minimal DAG, enforcing the ``compute-once'' guarantee regardless of the query source.
    
    \item \textbf{Adaptive Leaf Polarity:} To ensure the sparsity invariant holds even for high-frequency terms (e.g., stopwords), the engine checks the document frequency. If $|\mathcal{I}(t)| > \frac{|U|}{2}$, the engine generates a Negative response $\langle U \setminus \mathcal{I}(t), \texttt{NEG} \rangle$ instead of a dense Positive one. This guarantees that the materialized set for any leaf node never exceeds half the universe size, strictly enforcing the sparsity bounds from the start and minimizing the theoretical upper bound of $|U_{\mathit{active}}|$ defined in Theorem 4.2.

    %\item \textbf{Task-Level Parallelism:} Unlike stateful iterators which enforce a rigid sequential processing order, the DAG structure explicitly exposes the dependency graph. This allows a dynamic scheduler to identify and execute logical units in parallel whenever their dependencies are satisfied (e.g., computing disjoint sub-graphs concurrently), utilizing multi-core architectures to reduce wall-clock latency.
\end{itemize}


==> QueryTreePrompt.tex <==
\section{Query Tree Prompt}\label{secQueryTreePrompt}

We used the following prompt on ``Gemini 2.5 Pro" to build the query trees, presented in~\ref{subSecComplexQueries}:

\begin{verbatim}
**Your Role:** You are an expert query understanding system. Your task is to translate natural language user queries for songs into their optimal Boolean Query Tree representation for our search engine.

**System Overview**

1.  **Retrieval Engine:** We use a powerful retrieval engine that processes Boolean Query Trees.
    *   **Internal Nodes:** `AND`, `OR`, `NOT`.
    *   **Leaf Nodes:** Search terms (posting lists).

2.  **Corpus:** A large database of songs. Each song's metadata is a JSON object with keys like `Title`, `Artists`, `Lyrics`, `Album`, `Genres`, `Year`, `Decade`, `Moods`, etc.

3.  **Indexing:** We index unigrams in two ways:
    *   **Field-Qualified Terms:** The term is prefixed with its source field (e.g., `TITLE:hotel`, `ARTISTS:queen`). This is the most precise way to search.
    *   **Raw Tokens:** The term without any field context (e.g., `hotel`, `queen`). This searches across all text fields (`Title`, `Lyrics`, `Album`, etc.).

**Your Toolkit: Query Refinements**

You have access to a sophisticated set of query refinements. You must intelligently decide when and how to apply them to create the best query tree. Your available refinements include:

*   **Intent Classification:** Determine the user's primary intent. A query like "by Queen" implies a search in the `ARTISTS` field. "Songs about California" implies a search in the `TITLE` or `LYRICS` fields.
*   **Entity Linking & Synonym Expansion:** Recognize aliases, alternate names, and common abbreviations. For example, you should know that "Queen Bee" is a common nickname for "Beyoncé".
*   **Spelling Correction & Partial Matching:** Correct common misspellings. You can also use partial tokens if they are unambiguous or as a fallback (e.g., "ARTISTS:b" could be a fragment of "Beyoncé").
*   **Field Prioritization:** A match in a specific, relevant field (like `TITLE`) is generally better than a generic match. Your query tree should reflect this preference, typically by putting the more specific `AND` clause first inside an `OR` block.

**Output Format**

Represent the final query as a nested S-expression.
`OPERATOR(argument1, argument2, ...)`

---

**Examples**

**Example 1: A query focused on a title.**
*   **User Query:** `Songs about Hotel California`
*   **Analysis:** The user is almost certainly looking for the song with this exact title. The primary search should be in the `TITLE` field. A fallback to a general search is a good secondary option for recall.
*   **Boolean Tree:**
    ```
    OR(
      AND(
        "TITLE:hotel",
        "TITLE:california"
      ),
      AND(
        "hotel",
        "california"
      )
    )
    ```

**Example 2: A query with a known artist alias.**
*   **User Query:** `Songs by Queen Bee`
*   **Analysis:** The user specifies an artist. "Queen Bee" is a primary alias for Beyoncé. The system should also account for a literal interpretation ("Queen" and "Bee") and potential partial tokens as fallbacks.
*   **Boolean Tree:**
    ```
    OR(
      "ARTISTS:beyonce",
      AND(
        "ARTISTS:queen",
        "ARTISTS:bee"
      ),
      AND(
        "ARTISTS:queen",
        "ARTISTS:b"
      )
    )
    ```
\end{verbatim}

==> ScholarQueryTrees.tex <==
\section{Expressiveness of the LR Language in Practice}\label{secCaseStudy}
    Having formally established that our retrieval language \texttt{LR} captures the complexity class \texttt{P}, this section illustrates the practical consequences of this expressive power. We use the domain of academic literature retrieval to demonstrate how the theoretical property of P-completeness translates into the ability to answer sophisticated, logically precise queries that are challenging for standard retrieval systems.

    \subsection{Example Domain: Academic Search}
        We assume a standard inverted index built from a corpus of academic papers where documents are represented as structured data with fields like Title, Author, Year, etc. This field-aware tokenization (e.g., TITLE:effectiveness, AUTHOR:hinton) allows for the precise, targeted queries shown below. The translation from natural language to the corresponding Query DAGs was performed by an LLM to illustrate how a modern front-end can target our expressive backend.

    \subsection{Complex Queries }\label{subSecComplexQueries}
        This subsection presents several natural language queries and their corresponding Query DAGs, which were generated using Google's Gemini Pro to illustrate how a modern LLM can act as a sophisticated ``Query Understanding'' front-end.

%\clearpage
\onecolumn
\begin{table}
\caption{Examples of queries and their Query DAG.}
\label{tab:query_examples} 
 \begin{tabularx}{\linewidth}{
    |>{\hsize=.45\hsize}X|
    >{\hsize=.45\hsize}X|}
\hline
% --- TABLE CONTENT ---
% --- ROW 1 ---

\includegraphics[
width=0.45\linewidth,
height=4cm,
keepaspectratio,
]{q1}                  
&
\includegraphics[
width=0.45\linewidth,
height=4cm,
keepaspectratio,
]{q2}                  
\\

% --- ROW 2 ---
\textit{Papers by Maning} 
&
\textit{Show me papers by Geoffrey Hinton, but not his work on Boltzmann Machines.} 
\\
\hline

\includegraphics[
width=0.45\linewidth,
height=4cm,
keepaspectratio,
]{q3}                  
&
\includegraphics[
width=0.45\linewidth,
height=4cm,
keepaspectratio,
]{q4}                  
\\

\textit{Papers by both Gerard Salton and Karen Jones, but not if Stephen Robertson is also an author.} 
&
\textit{Give me NLP papers on either parsing or generation, but nothing about machine translation.}
\\
\hline
\includegraphics[
width=0.45\linewidth,
height=4cm,
keepaspectratio,
]{q5}                  
&
\includegraphics[
width=0.45\linewidth,
height=4cm,
keepaspectratio,
]{q6}
\\
\textit{Papers on using SVMs or Neural Networks, but not for medical imaging applications.} 
&
\textit{Papers from SIGIR in the early 2010s, but not by author C. Zhai.} 
\\

\hline
\multicolumn{2}{|l|}{\includegraphics[
width=0.90\linewidth,
height=4cm,
keepaspectratio,
]{q7}}     
\\ 
\multicolumn{2}{|p{\textwidth}|}{\textit{Recent papers from top-ranking conferences that are about tokenization approaches in building LLMs.}}
\\
\hline
\multicolumn{2}{|l|}{\includegraphics[
width=0.9\linewidth,
height=3cm,
keepaspectratio,
]{q8}}     
\\ 
\multicolumn{2}{|p{\textwidth}|}{\textit{Find papers that discuss either `transformers' or `graph neural networks', but not both in the same paper.} 
}
\\
\hline
\end{tabularx}
\end{table}
%\vspace{-0.5cm}

These examples effectively demonstrate the framework's capacity for complex logical reasoning, handling multiple inclusions and exclusions with precision. However, this is just one consequence of the P-completeness of LR. As established in our theoretical analysis, the ability to simulate any Boolean circuit means our framework's power is not limited to the logical DAGs shown here. It extends to the computational queries discussed previously, such as numerical comparisons (citation\_count > K) or thresholding (at least k of N authors), which can be compiled into circuit-like DAGs. Therefore, while embedding-based systems may struggle to even guarantee the logical correctness shown in Table~\ref{tab:query_examples}, our framework's formal grounding provides a provable guarantee for an entire class of tractable computations, from pure logic to complex arithmetic.


==> SkipToLeafNodes.tex <==
\section{Implementation of \texttt{SkipTo} For Leaf Nodes Using Skip Pointers}\label{secSkipToLeafNodes}

In \ref{subsubsecSkipTo}, we showed a basic implementation for \texttt{SkipTo}. Here we present a faster implementation for this function, specifically for leaf nodes, utilizing skip pointers for optimized traversal of posting lists.

\begin{algorithm}
\caption{SkipTo($n$, $d$)}\label{algSkipToForLeaf}
\begin{algorithmic}[1]
  \Function{SkipToForLeafNode}{$n$ }
    \While{$n.State.Ptr \ne nil \textbf{ and } n.\text{State.Ptr.ID} \le d$}
      \If{$n.State.Ptr.HasSkip \textbf{ and } n.State.Ptr.Skip.ID \le d$}
        \State $n.State.Ptr \leftarrow n.State.Ptr.Skip $
      \Else
        \State $n.State.Ptr \leftarrow n.State.Ptr.Next $
      \EndIf
    \EndWhile


    \If{$n\text{.State.Ptr} = nil$} 
      \State $n.\text{State.CurrentIDs} \leftarrow \Call{MakeInterval}{U+1, U+1}$
    \EndIf
  \EndFunction
  
 \end{algorithmic}
\end{algorithm}


==> Subtract.tex <==
\section{Subtract Function}\label{secSubtract}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
    \caption{Subtract}
    \label{algHelperFunctions}
    \begin{algorithmic}[1]
      \Function{Subtract}{$A, B$}
        \State $D=[]$
        \While{$\Call{HasNext}{A}$}
          \If{$A.Value = B.Value$}
            \State \Call{MoveForward}{A}
            \State \Call{MoveForward}{B}
            \State $\textbf{continue}$
          \EndIf
          \If{$A.Value < B.Value$}
            \State $\Call{Add}{D, A.Value}$
            \State \Call{MoveForward}{A}
            \State $\textbf{continue}$
          \EndIf
          \While{$B.Skip < A.Value$}
            \State $B \gets B.Skip$
          \EndWhile
          \While{$\Call{HasNext}{B} \text{ and } B.Next < A.Value$}
            \State $\Call{MoveNext}{B}$
          \EndWhile
          
        \EndWhile
      \EndFunction
      
    \end{algorithmic}
\end{algorithm}
\end{minipage}%

